High order maximum principle preserving finite volume method for convection dominated problems

In this paper, we investigate the application of the maximum principle preserving (MPP) parametrized flux limiters to the high order finite volume scheme with Runge-Kutta time discretization for solving convection dominated problems. Such flux limiter was originally proposed in [Xu, Math. Comp., 2013] and further developed in [Xiong et. al., J. Comp. Phys., 2013] for finite difference WENO schemes with Runge-Kutta time discretization for convection equations. The main idea is to limit the temporal integrated high order numerical flux toward a first order MPP monotone flux. In this paper, we generalize such flux limiter to high order finite volume methods solving convection-dominated problems, which is easy to implement and introduces little computational overhead. More importantly, for the first time in the finite volume setting, we provide a general proof that the proposed flux limiter maintains high order accuracy of the original WENO scheme for linear advection problems without any additional time step restriction. For general nonlinear convection-dominated problems, we prove that the proposed flux limiter introduces up to $O(\Delta x^3+\Delta t^3)$ modification to the high order temporal integrated flux in the original WENO scheme without extra time step constraint. We also numerically investigate the preservation of up to ninth order accuracy of the proposed flux limiter in a general setting. The advantage of the proposed method is demonstrated through various numerical experiments.

==> table.tex <==
\begin{table}\tiny
\noindent

\begin{tabular}{|c ||l |l |l |l |}
\hline
 $\mathbf{F}$ & $\Lambda_{L,i,j}^M$ & $\Lambda_{R,i,j}^M$ & $\Lambda_{D,i,j}^M$ & $\Lambda_{U,i,j}^M$ \\
\hline
$(-,-,-,-)$ & $1$ & $1$ & $1$ & $1$ \\
\hline
$(-,-,-,+)$ & $1$ & $1$ & $1$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i,j+\frac{1}{2}}})$ \\
\hline
$(-,-,+,-)$ & $1$ & $1$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i,j-\frac{1}{2}}})$ & $1$ \\
\hline
$(-,-,+,+)$ & $1$ & $1$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i,j-\frac{1}{2}}+F_{i,j+\frac{1}{2}}})$ & $\Lambda_{D,i,j}^M$ \\
\hline
$(-,+,-,-)$ & $1$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i+\frac{1}{2},j}})$ & $1$ & $1$ \\
\hline
$(-,+,-,+)$ & $1$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i+\frac{1}{2},j}+F_{i,j+\frac{1}{2}}})$ & $1$ & $\Lambda_{R,i,j}^M$ \\
\hline
$(-,+,+,-)$ & $1$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i+\frac{1}{2},j}+F_{i,j-\frac{1}{2}}})$ & $\Lambda_{R,i,j}^M$ & $1$ \\
\hline
$(-,+,+,+)$ & $1$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i+\frac{1}{2},j}+F_{i,j-\frac{1}{2}}+F_{i,j+\frac{1}{2}}})$ & $\Lambda_{R,i,j}^M$ & $\Lambda_{R,i,j}^M$ \\
\hline
$(+,-,-,-)$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i-\frac{1}{2},j}})$ & $1$ & $1$ & $1$ \\
\hline
$(+,-,-,+)$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i-\frac{1}{2},j}+F_{i,j+\frac{1}{2}}})$ & $1$ & $1$ & $\Lambda_{L,i,j}^M$ \\
\hline
$(+,-,+,-)$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i-\frac{1}{2},j}+F_{i,j-\frac{1}{2}}})$ & $1$ & $\Lambda_{L,i,j}^M$ & $1$ \\
\hline
$(+,-,+,+)$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i-\frac{1}{2},j}+F_{i,j-\frac{1}{2}}+F_{i,j+\frac{1}{2}}})$ & $1$ & $\Lambda_{L,i,j}^M$ & $\Lambda_{L,i,j}^M$ \\
\hline
$(+,+,-,-)$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i-\frac{1}{2},j}+F_{i+\frac{1}{2},j}})$ & $\Lambda_{L,i,j}^M$ & $1$ & $1$ \\
\hline
$(+,+,-,+)$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i-\frac{1}{2},j}+F_{i+\frac{1}{2},j}+F_{i,j+\frac{1}{2}}})$ & $\Lambda_{L,i,j}^M$ & $1$ & $\Lambda_{L,i,j}^M$ \\
\hline
$(+,+,+,-)$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i-\frac{1}{2},j}+F_{i+\frac{1}{2},j}+F_{i,j-\frac{1}{2}}})$ & $\Lambda_{L,i,j}^M$ & $\Lambda_{L,i,j}^M$ & $1$ \\
\hline
$(+,+,+,+)$ & $min(1,\frac{\Gamma_{i,j}^M}{F_{i-\frac{1}{2},j}+F_{i+\frac{1}{2},j}+F_{i,j-\frac{1}{2}}+F_{i,j+\frac{1}{2}}})$ & $\Lambda_{L,i,j}^M$ & $\Lambda_{L,i,j}^M$ & $\Lambda_{L,i,j}^M$ \\
\hline
\end{tabular}
\caption{The values for $\Lambda_{L,i,j}^M, \Lambda_{R,i,j}^M, \Lambda_{D,i,j}^M, \Lambda_{U,i,j}^M$.}
\label{Lambdasmax}
\end{table}

